Approaches to Interpreter Composition

In this paper, we compose six different Python and Prolog VMs into 4 pairwise compositions: one using C interpreters; one running on the JVM; one using meta-tracing interpreters; and one using a C interpreter and a meta-tracing interpreter. We show that programs that cross the language barrier frequently execute faster in a meta-tracing composition, and that meta-tracing imposes a significantly lower overhead on composed programs relative to mono-language programs.

==> table/cmpnoconvert-speedup.tex <==
{\small
\begin{tabular}{llrl}
\toprule
\multicolumn{1}{c}{VM}&Benchmark
& \multicolumn{2}{c}{$\frac{\mbox{\emph{Python}}\rightarrow\mbox{\emph{Prolog}}}{\mbox{\emph{Python}}\overset{nc}{\rightarrow}\mbox{\emph{Prolog}}}$}
\\
\midrule
\multirow{9}{*}{\swithon} & SmallFunc
& 2.397$\times$ & {\tiny$\pm 0.041$}
\\
 & Loop1Arg0Result
& 1.412$\times$ & {\tiny$\pm 0.022$}
\\
 & Loop1Arg1Result
& 1.391$\times$ & {\tiny$\pm 0.023$}
\\
 & NondetLoop1Arg1Result
& 2.846$\times$ & {\tiny$\pm 0.039$}
\\
 & TermConstruction
& 14.875$\times$ & {\tiny$\pm 0.137$}
\\
 & Lists
& 205.645$\times$ & {\tiny$\pm 1.914$}
\\
 & sat-models
& 24.749$\times$ & {\tiny$\pm 0.260$}
\\
 & tube
& 1.512$\times$ & {\tiny$\pm 0.014$}
\\
 & connect4
& 1.439$\times$ & {\tiny$\pm 0.016$}
\\
\midrule
\multirow{9}{*}{\swipy} & SmallFunc
& 5.158$\times$ & {\tiny$\pm 0.130$}
\\
 & Loop1Arg0Result
& 1.405$\times$ & {\tiny$\pm 0.026$}
\\
 & Loop1Arg1Result
& 1.363$\times$ & {\tiny$\pm 0.012$}
\\
 & NondetLoop1Arg1Result
& 4.124$\times$ & {\tiny$\pm 0.215$}
\\
 & TermConstruction
& 9.234$\times$ & {\tiny$\pm 0.249$}
\\
 & Lists
& 23.171$\times$ & {\tiny$\pm 0.653$}
\\
 & sat-models
& 6.388$\times$ & {\tiny$\pm 0.152$}
\\
 & tube
& 1.384$\times$ & {\tiny$\pm 0.009$}
\\
 & connect4
& 1.428$\times$ & {\tiny$\pm 0.017$}
\\
\midrule
\multirow{9}{*}{\unipycation} & SmallFunc
& 1.064$\times$ & {\tiny$\pm 0.102$}
\\
 & Loop1Arg0Result
& 1.872$\times$ & {\tiny$\pm 0.095$}
\\
 & Loop1Arg1Result
& 1.703$\times$ & {\tiny$\pm 0.005$}
\\
 & NondetLoop1Arg1Result
& 1.561$\times$ & {\tiny$\pm 0.017$}
\\
 & TermConstruction
& 7.437$\times$ & {\tiny$\pm 0.060$}
\\
 & Lists
& 4.615$\times$ & {\tiny$\pm 0.034$}
\\
 & sat-models
& 1.807$\times$ & {\tiny$\pm 0.104$}
\\
 & tube
& 2.073$\times$ & {\tiny$\pm 0.040$}
\\
 & connect4
& 1.339$\times$ & {\tiny$\pm 0.027$}
\\
\midrule
\multirow{9}{*}{\unipycation nocrosstracing} & SmallFunc
& 1.579$\times$ & {\tiny$\pm 0.035$}
\\
 & Loop1Arg0Result
& 1.724$\times$ & {\tiny$\pm 0.062$}
\\
 & Loop1Arg1Result
& 1.728$\times$ & {\tiny$\pm 0.040$}
\\
 & NondetLoop1Arg1Result
& 1.705$\times$ & {\tiny$\pm 0.018$}
\\
 & TermConstruction
& 7.710$\times$ & {\tiny$\pm 0.178$}
\\
 & Lists
& 4.456$\times$ & {\tiny$\pm 0.039$}
\\
 & sat-models
& 2.010$\times$ & {\tiny$\pm 0.130$}
\\
 & tube
& 2.371$\times$ & {\tiny$\pm 0.122$}
\\
 & connect4
& 1.515$\times$ & {\tiny$\pm 0.017$}
\\
\bottomrule
\end{tabular}
}

